Specification Generation for Neural Networks in Systems

Specifications - precise mathematical representations of correct domain-specific behaviors - are crucial to guarantee the trustworthiness of computer systems. With the increasing development of neural networks as computer system components, specifications gain more importance as they can be used to regulate the behaviors of these black-box models. Traditionally, specifications are designed by domain experts based on their intuition of correct behavior. However, this is labor-intensive and hence not a scalable approach as computer system applications diversify. We hypothesize that the traditional (aka reference) algorithms that neural networks replace for higher performance can act as effective proxies for correct behaviors of the models, when available. This is because they have been used and tested for long enough to encode several aspects of the trustworthy/correct behaviors in the underlying domain. Driven by our hypothesis, we develop a novel automated framework, SpecTRA to generate specifications for neural networks using references. We formulate specification generation as an optimization problem and solve it with observations of reference behaviors. SpecTRA clusters similar observations into compact specifications. We present specifications generated by SpecTRA for neural networks in adaptive bit rate and congestion control algorithms. Our specifications show evidence of being correct and matching intuition. Moreover, we use our specifications to show several unknown vulnerabilities of the SOTA models for computer systems.

==> Makefile <==
SHELL := /bin/bash
WORK := $(shell basename `pwd`)
MAIN = paper.tex

BASE := $(basename $(MAIN))
SRCEXT := $(patsubst $(BASE).%,%,$(MAIN))
BIBFILES := $(wildcard *.bib)
STYLINK := $(notdir $(wildcard *.sty))
STYFILES := $(sort $(STYLINK) $(wildcard *.sty))
TEXFILES := $(sort $(MAIN) $(wildcard *.tex) $(STYFILES))
# eval
PLOT_GRAPHS := $(wildcard eval/graphs/*.eps)
PLOT_SCRIPTS := $(wildcard eval/scripts/*.py)
PLOT_GNUPLOT := $(wildcard eval/scripts/*.gnu)
PLOT_GNUPLOT2 := $(wildcard eval/scripts/*.gnuplot)
RAWDATA := $(wildcard eval/raw/*)
EVAL_MAIN:=eval/main_eval.py

LATEX = pdflatex
BIBTEX = bibtex -min-crossrefs=1000
PS2PDF = ps2pdf


# by default, not extended mode
# change this to 1 if you want extended mode by default
EXTENDED ?= 0
ifeq ($(EXTENDED),1)
EXTDEF := \def\buildextended{}
else
EXTDEF := 
endif

# by default, editing marks
# change this to 0 if you want no edit marks by default
EDITING ?= 1
ifeq ($(EDITING),1)
EDITDEF := 
else
EDITDEF := \def\noeditingmarks{}
endif

all: $(BASE).pdf

# for appendix, tmp for submission
appendix: apppdf.ltx appendix.tex
	latexmk -pdf apppdf.ltx

#.headline:
#	$(MAKE) -C headline

#.images: headline/headline.eps  $(addsuffix /*.eps,$(IMAGES)) $(addsuffix /*.tex,$(IMAGES))
#	for i in $(IMAGES); do $(MAKE) -C $$i; done
#	touch $@

#graphs/%.pdf:
#	touch scripts/$(shell basename $@ .pdf).sh

%.pdf: %.eps
	perl -ne 'exit 1 unless /\n/' $< \
		|| perl -p -i -e 's/\r/\n/g' $<
	epstopdf --outfile=$@ $<

$(BASE).pdf: %.pdf: %.$(SRCEXT) $(TEXFILES) $(BIBFILES) $(PLOT_GRAPHS)
	@echo "BASE"
	@echo $?
	#@if [[ "$?" == *"$(EVAL_MAIN)"* ]]; then \
	#	python eval/main_eval.py ./eval/; \
	#fi
	$(eval LTXINPUT := "$(EXTDEF)$(EDITDEF)\input{$<}")
	latexmk -pdf $(MAIN)

%.pdf: %.ltx
	latexmk -pdf $<

$(PLOT_GRAPHS) : $(PLOT_SCRIPTS) $(PLOT_GNUPLOT) $(PLOT_GNUPLOT2) $(RAWDATA) 
	@echo "PLOT_GRAPHS"
	@echo $?
#	@python eval/main_eval.py ./eval/

# python:
# 	python eval/main_eval.py ./eval/

show: $(BASE).pdf
	xpdf -fullscreen $(BASE).pdf

osx: $(BASE).pdf
	open $(BASE).pdf

double:
	for i in $(TEXFILES); do perl double.pl $$i; done	

clean:
		rm -f eval/*.aux # eval/eval3table.tex eval/graphs/* eval/scripts/*.dat
		rm -f $(BASE).ps $(BASE).pdf
		rm -f *.dvi *.aux *.log *.bbl *.blg *.lof *.lot *.toc *.bak *.out .images *.fdb_latexmk *.fls
		for i in $(IMAGES); do $(MAKE) -C $$i clean; done


==> checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, the claims are substantiated in the experimental results. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have a separate limitations section.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our technical sections~\ref{sec:formal} and \ref{sec:implementation} provide those. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Given in the experimental section~\ref{sec:results}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The code is provided. We use open-source datasets. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide those in the experiments section~\ref{sec:results}. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our results are deterministic. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: In Section~\ref{sec:results}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We don't perceive any ethical violations. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss the positive impacts. We don't see any negative impacts of our work.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We don't have those artifacts. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide appropriate citations.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide the code with a readme on getting the results. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not do experiments involving humans. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No experiments involving humans
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> extras.tex <==
 Ideally, the users of the video streaming systems prefer a high bit rate of the video, minimum rebuffering, and minimum variation in the bit rate for subsequent steps. However, these desirable properties pose tradeoffs, such as a high bit rate may lead to high rebuffering in a network having low throughput. Thus, ABR algorithms optimize a Quality of Experience (QoE) metric that captures the overall performance of the video streaming system.

 Traditional ABR algorithms consist of heuristics to choose a bitrate, such as comparing the values of the buffer size and observed throughput history of the system with thresholds identified by domain experts and developing models of the system to predict future throughput values. Neural ABR algorithms, developed using Reinforcement Learning can maximize a given QoE objective with a learned agent. 

 % We use the DSL $\lang$ in~\eqref{eq:specDSL} to represent the set of specifications $\setspecs\in\lang$ as a conjunction of specifications $\spec$ defined over real numbers. Each $\spec$ consists of a precondition $\pre$ that implies a postcondition $\post$. $\pre$ gives real-valued bounds on each input feature variable $X[i]$ and $\post$ gives bounds on all the possible outputs with a given input $X$. 

% The capitalized symbols $\{L,R,L_1,R_1,\dots,L_\numinputs,R_\numinputs\}$ are constants in the DSL and $\{x_1,\dots,x_\numinputs,y\}$ are variables 
% \begin{equation}
%     \label{eq:specDSL}
%     \begin{split}
%         \setspecs &\Coloneqq \emptyset \mid \setspecs\cup\{\spec\}\\
%         \spec &\Coloneqq \pre\implies\post\\
%         \pre &\Coloneqq L_X\leq X\leq U_X\\
%         \post &\Coloneqq L_Y\leq Y\leq U_Y\\
%         X &\Coloneqq \realv[\numinputs]\\
%         Y &\Coloneqq \realv[\numoutputs]\\
%         v &\Coloneqq X \mid Y\\
%         L_v &\Coloneqq [c_1,\dots, c_i,\dots], c_i \in \mathbb{R}\\
%         U_v &\Coloneqq [c_1,\dots, c_i,\dots], c_i \in \mathbb{R}\\
%         \realv &\Coloneqq\mathbb{R}\\
%     \end{split}
% \end{equation}

==> intro.tex <==
\section{Introduction}
Neural networks are recently finding numerous applications as computer system
components~\citep{aurora,pensieve,decima,mendis2019ithemalaccurateportablefast}.
This is due to their high average performance and significantly lower
development overheads than the traditionally used algorithms/heuristics.
However, the widespread user-facing applications of computer systems require
them to maintain high standards of performance and reliability. Although neural
networks are optimized to exhibit higher average performance than any
traditionally used algorithms, they are recognized to be inherently
uninterpretable~\citep{comet} and hence not reliable for practical deployment.

Due to general concerns about the black-box nature of neural networks (NNs), there has been much interest in checking whether they satisfy desirable domain-specific properties~\cite{wu2022scalable, wei2023building,vnncomp23,domcons,verifying_learning_augmented_systems} beyond computer systems. For example, in the vision domain, a desirable property to check is that the classification output of NNs should not change under the rotation of the original image~\cite{YangLM023,deepg}. To enable automated verification, such properties are precisely described mathematically as \textit{specifications} characterizing desirable NN outputs corresponding to given inputs. 
Most existing works use manually-crafted specifications~\cite{verifying_learning_augmented_systems,vnncomp23,wu2022scalable,nn4sysbench}. There are two main issues with this approach --- (i) Manual specifications require significant domain knowledge and intuition which may not always be available. For example, it is unclear how to define the local perturbation region for robustness specifications for NN-based controllers in the systems domain without intervention of human experts~\cite{Chakravarthy2022PropertyDrivenEO}.  
(ii) Manually designed specifications may be incorrect and contain inputs on which the specification should not hold~\cite{frosst}. 
%Traditionally, neural network specifications have been on local robustness, fairness~\citep{fairnessSpec}, and other specifications that capture the general desirable properties for neural networks. However, these formal specifications do not capture the intuitive understanding of domain experts about the expected behaviors of neural networks as system components, verifying which can make the system more trustworthy for deployment. 

%Neural Networks have been developed to act as computer and communication system components by replacing traditional algorithms. For example, Pensieve~\citep{pensieve} is a deep neural network trained using reinforcement learning, to act as an Adaptive Bit Rate (ABR) algorithm in video streaming systems, that picks the bit rate at which the next video chunk should be fetched from a server to a client. The sequence of bit rate choices governs the performance of the video streaming system. 
%Pensieve is a better-performing alternative for several heuristic-based algorithms that have been manually designed based on the dynamics of the interaction of the network and video streaming systems and the intuition of domain experts. Popular traditional ABR algorithms are the buffer-based algorithm~\citep{bba} and the MPC algorithm~\citep{mpc}. The buffer-based algorithm selects bit rates based on buffer occupancy at any time step by binning the buffer size heuristically and assigning higher bit rates to bins with greater buffer sizes. The MPC algorithm makes a model of the observed throughput of the network to predict the throughput at the subsequent steps and optimize the performance based on the throughput prediction and the system state. Pensieve has been developed to deliver higher performance, however, it is unclear whether Pensieve can be reliably deployed in production. 
%The heuristic-driven algorithms, while less performant, are deemed trustworthy by domain experts as these exhibit behavior that conforms to the intuition of the experts. This suggests the need to verify whether the neural networks as computer system components also exhibit common behavior expected from them and can hence reliably substitute the traditional components. 
% This is not immediately clear, as neural networks are black boxes making it impossible to gauge their behavior automatically. 



\textbf{This work}. Contrary to manually-designed specifications, we develop a general framework to \textit{automatically} generate specifications for computer system domains. A special characteristic of computer systems is that several applications have traditionally-used rule-based algorithms and heuristics (a.k.a. references) which, even though not as performant as NNs, are trustworthy as they are designed according to the domain experts' intuitions of correct behavior and have been tested in production-level settings for long. We propose exploiting these artifacts of computer systems to automatically design specifications for NNs in these domains.
% Automated generation requires access to an oracle that can tell us what should be the DNN output on a given input. For the traditional vision and NLP domains, the oracles are humans and it is infeasible to get the expected output corresponding to all possible inputs. 
% Instead, we focus on domains where real-world reference implementations that are deemed trustworthy and safe by domain experts, are available. Examples include the systems, networking, and security domains~\cite{pensieve,aurora,mpc,bba,Chen0QLJW21}. 
We use the outputs of the references to automatically generate specifications for their NN counterparts.

%We focus on domains where DNNs have been proposed to replace traditional algorithms. Examples include congestion control and video streaming~\cite{pensieve,mpc,aurora}.   

%identify the properties expected of neural networks in domains where . These specifications can be verified in neural networks post-training and before deployment.

\textbf{Key challenges}. First, several traditional implementations exist for the same application, e.g., for adaptive bit rate~\cite{mpc,bba}. These implementations can have diverging behaviors on the same input. It is unclear how to combine such diverse feedback into specifications for the NN. Second, the set of specifications corresponding to references is not unique. Some specifications are more useful than others. So we need to design criteria to identify \textit{high quality} specifications. Finally, we need to design algorithms that can synthesize the specifications with the desired traits. 


%Traditional implementations are complex and contain thousands of lines of intricate low-level code. 


%It is difficult to express the intuitive understanding of domain experts in a formal language to be amenable to verification. Firstly, specifications should capture behavior commonly anticipated by several domain experts, obtaining the data for which requires significant human effort. Secondly, it is unclear how to efficiently and automatically present the data as a few important specifications that can be verified by contemporary neural network verification systems and make the verified neural networks trustworthy. 

\textbf{Our approach}. We propose an automated specification generation method for domains where references are available. Our specifications are based on pre and postconditions consisting of constraints on the NN inputs and outputs respectively~\cite{hoare:69}. We require that if the NN input satisfies the precondition then its output must satisfy the postcondition. %The postcondition is constructed by combining the output of multiple references.    
We formalize the desired traits that useful specifications should satisfy and pose their generation as an optimization problem (Section~\ref{sec:formal}). We design an effective algorithm, called \tool{},  based on clustering for solving the optimization problem. Our algorithm does not require white-box access, therefore our algorithm can handle references that have complicated implementations or whose source code is unavailable. We generate expressive and reliable\todo{define reliability of specs} specifications for NNs in two challenging and practically important domains: congestion control~\cite{aurora} and adaptive bit rate for video streaming~\cite{pensieve}.
Besides being useful for testing and verification, our specifications can serve as concise, interpretable descriptions of desirable behaviors in the chosen domain. 

%study the execution traces of several traditional algorithms a.k.a \emph{references} and derive their collective behaviors as those that conform to the intuition of the domain experts who designed the references. The availability of references is a convenient characteristic of the computer systems domain, that we exploit for making trustworthy and high-performing neural components.

%We then mine \emph{likely} specifications from the collective behavior patterns. We optimize the specifications to be few and accurately represent the maximum salient features common across multiple references, as observed in the execution traces. The specifications are mined in a specification language that can be easily converted to VNN-Lib~\citep{vnn-lib} --- the standard for expressing specifications for neural network verification.

\textbf{Contributions}. Our main contributions are: 
\begin{enumerate}
    \item We formalize the generation of expressive and reliable specifications from references as an optimization problem. 
    \item We develop an automated specification mining algorithm, called \tool{}\footnote{\textbf{Spec}ifications from \textbf{T}rustworthy \textbf{R}eference \textbf{A}lgorithms}, based on our formalism that can handle complicated and closed-sourced reference implementations. 
    \item We create specifications for NNs for Adaptive Bitrate and congestion control applications. We demonstrate the accuracy\todo{need to define accuracy, as it is not a common term here} of our specifications and also the necessity of our specifications for good performance. 
\end{enumerate}


==> limitations.tex <==
% \section{Limitations and Future work} 

%creates spec on the available data
%does not scale to high-dimensional 

==> notes.tex <==
\begin{itemize}
    \item Data-driven, so fewer dimensions is better. 
    \item 
\end{itemize}
